Output-Feedback System Level Synthesis via Dynamic Programming

System Level Synthesis (SLS) allows us to construct internally stabilizing controllers for large-scale systems. However, solving large-scale SLS problems is computationally expensive and the state-of-the-art methods consider only state feedback; output feedback poses additional challenges because the constraints are no longer uniquely row or column separable. We exploit the structure of the output-feedback SLS problem by vectorizing the multi-sided matrix multiplications in the SLS optimization constraints, which allows us to reformulate it as a discrete-time control problem and solve using two stages of dynamic programming (DP). Additionally, we derive an approximation algorithm that offers a faster runtime by partially enforcing the constraints, and show that this algorithm offers the same results. DP solves SLS up to $7$ times faster, with an additional 42% to 68% improvement using the approximation algorithm, than a convex program solver, and scales with large state dimensions and finite impulse response horizon.

==> figures/draw/patterns.tex <==
\definecolor{Darkgreen}{HTML}{008000}
\definecolor{EdgeGrey}{HTML}{7F7F7F}

\definecolor{color_o}{RGB}{  0,  0,  0}
\definecolor{color_l}{RGB}{240, 30, 30}
\definecolor{color_i}{RGB}{  0,180, 80}
\definecolor{color_n}{RGB}{ 80,130,190}
\definecolor{color_v}{RGB}{240,150, 30}
\definecolor{color_a}{RGB}{190,130, 80}
\definecolor{color_r}{RGB}{130, 80,190}

\pgfdeclarepatternformonly{pattern_o}
{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{2.5pt}{2.5pt}} % lowerleft,upperright
{\pgfqpoint{3pt}{3pt}}%
{
  \pgfusepath{fill}
}
\pgfdeclarepatternformonly{pattern_l}
{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{7pt}{3pt}} % lowerleft,upperright
{\pgfqpoint{7pt}{3pt}}%
{
  \pgfsetlinewidth{0.2pt}
  \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
  \pgfpathlineto{\pgfqpoint{7.7pt}{3.3pt}}
  \pgfusepath{stroke}
}
\pgfdeclarepatternformonly{pattern_i}
{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{2.5pt}{2.5pt}} % lowerleft,upperright
{\pgfqpoint{3pt}{3pt}}%
{
  \pgfpathcircle{\pgfqpoint{0pt}{0pt}}{.5pt}
  \pgfpathcircle{\pgfqpoint{1.5pt}{1.5pt}}{.5pt}
  \pgfusepath{fill}
}
\pgfdeclarepatternformonly{pattern_n}
{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{6pt}{4pt}} % lowerleft,upperright
{\pgfqpoint{6pt}{4pt}}%
{
  \pgfsetlinewidth{0.2pt}
  \pgfpathmoveto{\pgfqpoint{0pt}{4pt}}
  \pgfpathlineto{\pgfqpoint{6pt}{0pt}}
  \pgfusepath{stroke}
}
\pgfdeclarepatternformonly{pattern_v}
{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{6pt}{6pt}} % lowerleft,upperright
{\pgfqpoint{5pt}{5pt}}%size
{
  \pgfsetlinewidth{0.2pt}
  \pgfpathmoveto{\pgfqpoint{5pt}{0pt}}
  \pgfpathlineto{\pgfqpoint{0pt}{5pt}}
  \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
  \pgfpathlineto{\pgfqpoint{5pt}{5pt}}
  \pgfusepath{stroke}
}
\pgfdeclarepatternformonly{pattern_a}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{6pt}{6pt}}{\pgfqpoint{6pt}{6pt}}%
{
  \pgfsetlinewidth{0.2pt}
  \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
  \pgfpathlineto{\pgfqpoint{6pt}{6pt}}
  \pgfusepath{stroke}
  \pgfpathcircle{\pgfqpoint{4.5pt}{1.5pt}}{.5pt}
  \pgfpathcircle{\pgfqpoint{1.5pt}{4.5pt}}{.5pt}
  \pgfusepath{fill}
}
\pgfdeclarepatternformonly{pattern_r}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{4pt}{4pt}}{\pgfqpoint{4pt}{4pt}}%
{
  \pgfsetlinewidth{0.2pt}
  \pgfpathcircle{\pgfqpoint{1.5pt}{1.5pt}}{1pt}
  \pgfusepath{stroke}
}

